REPLUG: Retrieval-Augmented Black-Box Language Models

We introduce REPLUG, a retrieval-augmented language modeling framework that treats the language model (LM) as a black box and augments it with a tuneable retrieval model. Unlike prior retrieval-augmented LMs that train language models with special cross attention mechanisms to encode the retrieved text, REPLUG simply prepends retrieved documents to the input for the frozen black-box LM. This simple design can be easily applied to any existing retrieval and language models. Furthermore, we show that the LM can be used to supervise the retrieval model, which can then find documents that help the LM make better predictions. Our experiments demonstrate that REPLUG with the tuned retriever significantly improves the performance of GPT-3 (175B) on language modeling by 6.3%, as well as the performance of Codex on five-shot MMLU by 5.1%.

==> table/pile.tex <==
\begin{table*}[h]
\small
 % \addtolength{\tabcolsep}{-1pt} 
\centering
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{3}{c}{Davinci (175B)} & \multicolumn{3}{c}{Curie (6.7B)} \\
\cmidrule(lr){2-4}
\cmidrule(lr){5-7}
Subset & Original &  + contriever &  + \model\ & Original & + contriever &  + \textsc{RE-Plug} \\
\midrule
% & Original &  contriever &  \model\ & Original &  contriever & \model \\
ArxiV & 0.77 & 0.74 & 0.73 & 0.85 & 0.83 & 0.80 \\
Books3 & 0.71 & 0.69 & 0.68 & 0.83 & 0.82 & 0.80 \\
DM Math & 2.00 & 1.97 & 1.74 & 2.11 & 2.09 & 2.06 \\
Freelaw & 0.60 & 0.57 & 0.55 & 0.67 & 0.65 & 0.62 \\
GitHub & 0.56 & 0.41 & 0.44 & 0.64 & 0.58 & 0.45 \\
Gutenberg & 0.71 & 0.48 & 0.70 & 0.79 & 0.70 & 0.53 \\
Hackernews & 0.95 & 0.90 & 0.92 & 1.02 & 1.00 & 0.95 \\
NIH Exporter & 0.62 & 0.61 & 0.60 & 0.68 & 0.67 & 0.65 \\
Open Subtitles & 0.91 & 0.91 & 0.89 & 0.99 & 0.98 & 0.99 \\
Phil Papers & 0.81 & 0.80 & 0.74 & 0.88 & 0.88 & 0.86 \\
PileCC & 0.71 & 0.67 & 0.64 & 0.78 & 0.77 & 0.72 \\
Pubmed Abstracts & 0.62 & 0.61 & 0.59 & 0.68 & 0.67 & 0.65 \\
Pubmed Central & 0.65 & 0.57 & 0.59 & 0.72 & 0.68 & 0.61 \\
StackExchange & 0.73 & 0.73 & 0.72 & 0.80 & 0.80 & 0.84 \\
Ubuntu IRC & 0.99 & 0.95 & 0.94 & 1.10 & 1.08 & 1.04 \\
USPTO & 0.53 & 0.51 & 0.51 & 0.58 & 0.57 & 0.54 \\
\midrule
Avg. & 0.80 & 0.76 &\textbf{0.75}& 0.88 & 0.86 & \textbf{0.82} \\
\bottomrule
\end{tabular}
\caption{BPB on the Pile} \weijia{only report the avergae: three numbers but with different models}
\label{tab:main}
\end{table*}

